Generalisations of the Laplace-Runge-Lenz vector

The characteristic feature of the Kepler Problem is the existence of the so-called Laplace--Runge--Lenz vector which enables a very simple discussion of the properties of the orbit for the problem. It is found that there are many classes of problems, some closely related to the Kepler Problem and others somewhat remote, which share the possession of a conserved vector which plays a significant r\^ole in the analysis of these problems.

==> leach-commands.tex <==
% This command footnotes by symbols
 \renewcommand{\thefootnote}{\fnsymbol{footnote}}

\catcode`\@=11
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\@addtoreset{equation}{section}
\catcode`\@=10


% ** Definitions **
\def\dsp{\displaystyle}
\def\d{\mbox{\rm d}}
\def\e{\mbox{\rm e}}

%    ** math **

\def\ut#1{{\mathunderaccent\tilde #1}}
\def\cosec{{\rm cosec}}
\def\arcsec{{\rm arcsec}}
\def\kd{{\delta _{ij}}}
\def\ke{{\epsilon _{ijk}}}

\def\half{\mbox{$\frac{1}{2}$}}

\def\ha{\mbox{$\frac{1}{2}$}}
\def\tha{\mbox{$\frac{3}{2}$}}
\def\fha{\mbox{$\frac{5}{2}$}}
\def\nha{\mbox{$\frac{n}{2}$}}
\def\oei{\mbox{$\frac{1}{8}$}}
\def\tei{\mbox{$\frac{3}{8}$}}
\def\oqr{\mbox{$\frac{1}{4}$}}
\def\tqr{\mbox{$\frac{3}{4}$}}
\def\otw{\mbox{$\frac{1}{12}$}}
\def\oth{\mbox{$\frac{1}{3}$}}
\def\tth{\mbox{$\frac{2}{3}$}}
\def\fth{\mbox{$\frac{4}{3}$}}
\def\ofi{\mbox{$\frac{1}{5}$}}
\def\osi{\mbox{$\frac{1}{6}$}}
\def\fei{\mbox{$\frac{5}{8}$}}
\def\fra#1#2{\mbox{$\frac{#1}{#2}$}}
\def\f{\frac}
\def\p{\dsp\partial}
\def\arcsinh{{\rm arcsinh}}
\def\sinh{{\rm sinh}}
\def\cosh{{\rm cosh}}
\def\arccosh{{\rm arccosh}}
\def\arctanh{{\rm arctanh}}
\def\tanh{{\rm tanh}}
\def\coth{{\rm coth}}
\def\sech{{\rm sech}}
\def\cosech{{\rm cosech}}

%    ** greek **

\def\ga{\alpha}
\def\gb{\beta}
\def\gc{\chi}
\def\gd{\delta}
\def\ge{\epsilon}
\def\gf{\phi}
\def\gg{\gamma}
\def\gi{\iota}
\def\gk{\kappa}
\def\gl{\lambda}
\def\gp{\psi}
%\def\gr{\rho}
\def\gs{\sigma}
\def\gt{\theta}
\def\gu{\upsilon}
\def\gve{\varepsilon}
\def\gw{\omega}
\def\gz{\zeta}
\def\gG{\Gamma}
\def\gD{\Delta}
\def\gF{\Phi}
\def\gL{\Lambda}
\def\gP{\Psi}
%\def\gR{\Rho}
\def\gS{\Sigma}
\def\gT{\Theta}
\def\gW{\Omega}

\def\bhw{\hat{\mbox{\boldmath $\omega$}}}
\def\bht{\hat{\mbox{\boldmath $\theta$}}}
\def\bhf{\hat{\mbox{\boldmath $\phi$}}}
\def\bhi{\hat{\mbox{\bfseries \itshape \i}}}
\def\bhj{\hat{\mbox{\bfseries \itshape \j}}}

%reserve variants
%\def\bhi{\hat{\mbox{\boldmath $i$}}}
%\def\bhj{\hat{\mbox{\boldmath $j$}}}

%authors variants
%\def\bhi{\hat{\mbox{\boldmath $\i$}}}
%\def\bhj{\hat{\mbox{\boldmath $\j$}}}

\def\mbt{\mbox{\boldmath $\theta$}}
\def\bhr{\hat{\mbox{\boldmath $r$}}}
\def\bhL{\hat{\mbox{\boldmath $L$}}}


\def\bfA{{\mbox{\boldmath $A$}}}
\def\bfE{{\mbox{\boldmath $E$}}}
\def\bfF{{\mbox{\boldmath $F$}}}
\def\bfI{{\mbox{\boldmath $I$}}}
\def\bfJ{{\mbox{\boldmath $J$}}}
\def\bfK{{\mbox{\boldmath $K$}}}
\def\bfL{{\mbox{\boldmath $L$}}}
\def\bfM{{\mbox{\boldmath $M$}}}
\def\bfN{{\mbox{\boldmath $N$}}}
\def\bfP{{\mbox{\boldmath $P$}}}
\def\bfS{{\mbox{\boldmath $S$}}}
\def\bfe{{\mbox{\boldmath $e$}}}
\def\bff{{\mbox{\boldmath $f$}}}
\def\bfk{{\mbox{\boldmath $k$}}}
\def\bfp{{\mbox{\boldmath $p$}}}
\def\bfr{{\mbox{\boldmath $r$}}}
\def\bft{{\mbox{\boldmath $t$}}}
\def\bfu{{\mbox{\boldmath $u$}}}
%    ** differentials **

\def\p{\dsp \partial}

% \def\pa{{\p\over\p a}}
\def\pb{{\p\over\p b}}
\def\pc{{\p\over\p c}}
\def\pd{{\p\over\p d}}
\def\pe{{\p\over\p e}}
\def\pf{{\p\over\p f}}
\def\pg{{\p\over\p g}}
\def\ph{{\p\over\p h}}
%\def\pi{{\p\over\p i}}
\def\pj{{\p\over\p j}}
\def\pk{{\p\over\p k}}
\def\pl{{\p\over\p l}}
% \def\pm{{\p\over\p m}}
\def\pn{{\p\over\p n}}
\def\po{{\p\over\p o}}
% \def\pp{{\p\over\p p}}
\def\pq{{\p\over\p q}}
\def\pr{{\p\over\p r}}
\def\ps{{\p\over\p s}}
\def\pt{{\p\over\p t}}
\def\pu{{\p\over\p u}}
\def\pv{{\p\over\p v}}
\def\pw{{\p\over\p w}}
\def\px{{\p\over\p x}}
\def\py{{\p\over\p y}}
\def\pz{{\p\over\p z}}

\def\upq{\partial_q}
\def\upr{\partial_r}
\def\upt{\partial_t}
\def\upu{\partial_u}
\def\upv{\partial_v}
\def\upx{\partial_x}
\def\upy{\partial_y}
\def\upz{\partial_z}
\def\up#1{\partial_{#1}}

\def\pA{{\p\over\p A}}
\def\pB{{\p\over\p B}}
\def\pC{{\p\over\p C}}
\def\pD{{\p\over\p D}}
\def\pE{{\p\over\p E}}
\def\pF{{\p\over\p F}}
\def\pG{{\p\over\p G}}
\def\pH{{\p\over\p H}}
\def\pI{{\p\over\p I}}
\def\pJ{{\p\over\p J}}
\def\pK{{\p\over\p K}}
\def\pL{{\p\over\p L}}
\def\pM{{\p\over\p M}}
\def\pN{{\p\over\p N}}
\def\pO{{\p\over\p O}}
%\def\pP{{\p\over\p P}}
\def\pQ{{\p\over\p Q}}
\def\pR{{\p\over\p R}}
\def\pS{{\p\over\p S}}
\def\pT{{\p\over\p T}}
\def\pU{{\p\over\p U}}
\def\pV{{\p\over\p V}}
\def\pW{{\p\over\p W}}
\def\pX{{\p\over\p X}}
\def\pY{{\p\over\p Y}}
\def\pZ{{\p\over\p Z}}

\def\da{{\d\over\d a}}
\def\db{{\d\over\d b}}
\def\dc{{\d\over\d c}}
% \def\dd{{\d\over\d d}}
\def\de{{\d\over\d e}}
\def\df{{\d\over\d f}}
\def\dg{{\d\over\d g}}
\def\dh{{\d\over\d h}}
\def\di{{\d\over\d i}}
\def\dj{{\d\over\d j}}
\def\dk{{\d\over\d k}}
\def\dl{{\d\over\d l}}
% \def\dm{{\d\over\d m}}
\def\dn{{\d\over\d n}}
\def\do{{\d\over\d o}}
\def\ddp{{\d\over\d p}}
\def\dq{{\d\over\d q}}
\def\dr{{\d\over\d r}}
\def\ds{{\d\over\d s}}
\def\dt{{\d\over\d t}}
\def\du{{\d\over\d u}}
\def\dv{{\d\over\d v}}
\def\dw{{\d\over\d w}}
\def\dx{{\d\over\d x}}
\def\dy{{\d\over\d y}}
\def\dz{{\d\over\d z}}

\def\dA{{\d\over\d A}}
\def\dB{{\d\over\d B}}
\def\dC{{\d\over\d C}}
\def\dD{{\d\over\d D}}
\def\dE{{\d\over\d E}}
\def\dF{{\d\over\d F}}
\def\dG{{\d\over\d G}}
\def\dH{{\d\over\d H}}
\def\dI{{\d\over\d I}}
\def\dJ{{\d\over\d J}}
\def\dK{{\d\over\d K}}
\def\dL{{\d\over\d L}}
\def\dM{{\d\over\d M}}
\def\dN{{\d\over\d N}}
\def\dO{{\d\over\d O}}
\def\dP{{\d\over\d P}}
\def\dQ{{\d\over\d Q}}
\def\dR{{\d\over\d R}}
\def\dS{{\d\over\d S}}
\def\dT{{\d\over\d T}}
\def\dU{{\d\over\d U}}
\def\dV{{\d\over\d V}}
\def\dW{{\d\over\d W}}
\def\dX{{\d\over\d X}}
\def\dY{{\d\over\d Y}}
\def\dZ{{\d\over\d Z}}


%    ** derivatives **

\def\pa#1#2{\f{\dsp \p#1}{\dsp \p#2}}
\def\pp#1#2{\f{\dsp \p^2 #1}{\dsp \p #2^2}}
\def\pam#1#2#3{\f{\dsp \p^2 #1}{\dsp \p #2 \p #3}}

\def\dm#1#2{\f{\dsp \d #1}{\dsp \d #2}}
\def\dd#1#2{\f{\dsp \d^2 #1}{\dsp \d #2^2}}

\def\dddot#1{\mathinner{\buildrel\vbox{\kern5pt\hbox{...}}\over{#1}}}

%    ** math misc **

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bq{\begin{eqnarray}}
\def\eq{\end{eqnarray}}
\def\beq{\begin{eqnarray*}}
\def\eeq{\end{eqnarray*}}
\def\ext#1#2{G^{[#1]} #2_{|_{\!\!|_{#2=0}}} = 0}
\def\exta#1{G^{[#1]}}
\def\extb#1#2{G^{[#1]} #2_{|_{\!\!|_{#2=0}}} }
\def\enter{$\longleftarrow\!\!\!^|$}
%   ** really misc **

\def\orl{Orl\'{e}ans}
\def\cf{{\it cf }}
\def\re#1{(\ref{#1})}
\def\ie{{\it ie }}
\def\eg{{\it eg }}
\def\viz{{\it videlicet }}
\def\etal{{\it et al }}
\def\n{\nonumber}
\def\({\left (}
\def\){\right )}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\z{&=&}
\def\lb{\left[ }
\def\rb{\right] }

